Pixel2Mesh: Generating 3D Mesh Models from Single RGB Images

We propose an end-to-end deep learning architecture that produces a 3D shape in triangular mesh from a single color image. Limited by the nature of deep neural network, previous methods usually represent a 3D shape in volume or point cloud, and it is non-trivial to convert them to the more ready-to-use mesh model. Unlike the existing methods, our network represents 3D mesh in a graph-based convolutional neural network and produces correct geometry by progressively deforming an ellipsoid, leveraging perceptual features extracted from the input image. We adopt a coarse-to-fine strategy to make the whole deformation procedure stable, and define various of mesh related losses to capture properties of different levels to guarantee visually appealing and physically accurate 3D geometry. Extensive experiments show that our method not only qualitatively produces mesh model with better details, but also achieves higher 3D shape estimation accuracy compared to the state-of-the-art.

==> tex/apped.tex <==



This document contains more comparison with other related methods and ablation study.

% \section{Extra results}

%\subsection{Results using real-world images}
%We have also evaluated our network using real-world images from the PSCAL VOC 2012 \cite{Everingham2010} dataset; the corresponding 3D models are from the PASCAL 3D+ dataset \cite{XiangMS14}.
%\todo{fine-tune?}

%\subsection{Comparison with Kar \etal \cite{KarTCM15}}

\begin{table}[h]
\centering
\setlength{\tabcolsep}{0.85mm}
\renewcommand{\arraystretch}{1.2}
\small
\begin{tabular}{@{}lrrrrrrrr@{}}
\hline
  % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
  Category & \multicolumn{4}{@{}c@{}}{Cai \etal \cite{CaiGLWMZ16}} & \multicolumn{4}{@{}c@{}}{Ours}\\
  \cmidrule(lr){2-5} \cmidrule(lr){6-9}
  Threshold & $0.5\tau$ & $\tau$ & $1.5\tau$ & $2\tau$ & $0.5\tau$ & $\tau$ & $1.5\tau$ & $2\tau$\\
\hline
\hline
  plane & 24.95 & 41.67 & 53.99 & 63.39 & \bfseries59.63 & \bfseries79.32 & \bfseries86.38 & \bfseries89.93\\
  bench & 21.78 & 34.24 & 42.39 & 48.84 & \bfseries41.88 & \bfseries60.63 & \bfseries70.04 & \bfseries75.84\\
  cabinet & 33.59 & 50.18 & 58.84 & 65.01 & \bfseries51.02 & \bfseries72.77 & \bfseries83.00 & \bfseries86.77\\
  car & 24.55 & 38.22 & 57.78 & 65.06 & \bfseries49.53 & \bfseries71.82 & \bfseries82.90 & \bfseries87.19\\
  chair & 27.54 & 40.24 & 48.57 & 55.04 & \bfseries39.92 &\bfseries 58.94 & \bfseries68.72 & \bfseries74.79\\
  monitor & 22.67 & 34.45 & 42.08 & 48.09 & \bfseries38.43 & \bfseries57.36 & \bfseries66.98 & \bfseries72.93\\
  lamp & 21.15 & 32.36 & 39.17 & 44.32 & \bfseries31.99 & \bfseries48.71 & \bfseries58.28 & \bfseries64.65\\
  speaker & 30.27 & 45.41 & 52.40 & 57.90 & \bfseries37.81 & \bfseries56.03 & \bfseries66.34 & \bfseries72.82\\
  firearm & 17.63 & 28.98 & 38.83 & 47.92 & \bfseries53.62 & \bfseries73.96 & \bfseries82.46 & \bfseries87.06\\
  couch & 25.11 & 40.26 & 47.68 & 53.53 & \bfseries43.32 & \bfseries65.04 & \bfseries76.04 & \bfseries82.21\\
  table & 30.03 & 44.13 & 52.90 & 59.69 & \bfseries52.25 & \bfseries70.19 & \bfseries78.27 & \bfseries82.98\\
  cellphone & 27.16 & 42.63 & 53.66 & 61.00 & \bfseries42.32 & \bfseries60.96 & \bfseries90.55 & \bfseries93.88\\
  watercraft & 24.79 & 37.51 & 45.89 & 52.34 & \bfseries41.10 & \bfseries62.08 & \bfseries72.49 & \bfseries 78.64\\
\hline
  mean & 25.48 & 39.25 & 48.78 & 55.55 & \bfseries44.83 & \bfseries64.43 & \bfseries75.57 & \bfseries80.74 \\
\hline
\end{tabular}
\vspace{3mm}
\caption{F-score (\%) on the ShapeNet test set at different thresholds, where $\tau=10^{-4}$. Larger is better. Best results under each threshold are bolded.}
\label{tab:res_refine}
\end{table}

\section{Comparison with mesh refinement}
Our method takes an initial mesh model and refine it with more details through a graphical CNN.
It is essentially a mesh refinement method.
We find that there are many previous work addressing this problem using non-learning based methods, and here we provide a comparison of this kind.

We compare with a recent mesh refinement method proposed by Cai \etal \cite{CaiGLWMZ16}. 
This method receives an initial mesh as input and aims to produce a refined mesh. 
%Since it does not incorporate more information into the mesh refinement procedure, one should not expect it to get better results. 
The comparison is reported in Table \ref{tab:res_refine}.
As can be seen, our method significantly outperforms Cai \etal in terms of F-score for occupancy accuracy.
It is expected since our network learns to extract information from the color image as the guidance to refine mesh instead of local smoothness.

\begin{figure}[t]
\centering
\includegraphics[width=1\linewidth]{figures/supp_figure1.pdf}
\caption{Correction of Figure 1 in paper.}
\label{fig:figure_1}
\end{figure}

\section{More qualitative results}
Figure 1,6 in our paper show a small number of our results and comparison to other methods.
Here we show more of that kind in Figure \ref{fig:supp_res}.
As can be seen, our results are significantly better than the others.


%\section{Qualitative Ablation Study}
%Figure 5 shows two examples of results of our system by disabling some major components.
%We show more visualization of ablation study in Figure \ref{xxx}.

\section{Correction of Figure 1 and 5}
Figure 1 and 5 in our paper shows our reconstructed mesh on 5 testing images.
However, we used the wrong figures for our final results.
The correct figures are shown in Figure \ref{fig:figure_1} and Figure \ref{fig:figure_5}.
It is true that our result does not contain details as much as the figure shown originally in paper, but our results still contain significantly more details compared to point cloud and volumetric representation.
Besides, all the numeric evaluations are correct, and none of the conclusion has been changed.
We are sorry for the confusion.

\begin{figure*}[t]
\centering
\includegraphics[width=0.98\linewidth]{figures/supp_figure5.pdf}
%\vspace{-3mm}
\caption{Correction of Figure 5 in paper.}
\label{fig:figure_5}
\end{figure*}

\begin{figure*}[t]
\centering
\includegraphics[width=0.99\linewidth]{figures/supp_res.pdf}
%\vspace{-3mm}
\caption{More qualitative results showing the point clouds and meshes of different methods.}
\label{fig:supp_res}
\end{figure*}
